Provable Self-Play Algorithms for Competitive Reinforcement Learning

Self-play, where the algorithm learns by playing against itself without requiring any direct supervision, has become the new weapon in modern Reinforcement Learning (RL) for achieving superhuman performance in practice. However, the majority of exisiting theory in reinforcement learning only applies to the setting where the agent plays against a fixed environment; it remains largely open whether self-play algorithms can be provably effective, especially when it is necessary to manage the exploration/exploitation tradeoff. We study self-play in competitive reinforcement learning under the setting of Markov games, a generalization of Markov decision processes to the two-player case. We introduce a self-play algorithm---Value Iteration with Upper/Lower Confidence Bound (VI-ULCB)---and show that it achieves regret $\tilde{\mathcal{O}}(\sqrt{T})$ after playing $T$ steps of the game, where the regret is measured by the agent's performance against a \emph{fully adversarial} opponent who can exploit the agent's strategy at \emph{any} step. We also introduce an explore-then-exploit style algorithm, which achieves a slightly worse regret of $\tilde{\mathcal{O}}(T^{2/3})$, but is guaranteed to run in polynomial time even in the worst case. To the best of our knowledge, our work presents the first line of provably sample-efficient self-play algorithms for competitive reinforcement learning.

==> Sections_arXiv/proof_poly_backup.tex <==
%!TEX root = ../two-player.tex
\section{Proof of Theorem \ref{thm:polytime_guarantee}}


\begin{align*}
\text{WEAKREGRET} = & \max_{\mu} \sum_{t}V^{\mu, \nu_t}(s_1) - \min_{\nu} \sum_{t} V^{\mu_t, \nu}(s_1)\\
= & \underbrace{\max_{\mu} \sum_{t} V^{\mu, \nu_t}(s_1) - \sum_{t} V^{\mu_t, \nu_t}(s_1)}_{\text{regret of max-player}} 
+ \underbrace{\sum_{t}V^{\mu_t, \nu_t}(s_1) - \min_{\nu}\sum_{t} V^{\mu_t, \nu}(s_1)}_{\text{regret of min-player}}
\end{align*}


\label{appendix:proof-polytime_guarantee}

First, we argue that WLOG we can consider the initial state as
fixed. Indeed, if the initial state is not fixed and (potentially)
adversarily chosen, we can treat different 
inital states as completely different games, which will at most
blow up the regret by a $S$ factor.
% a $\sqrt{S}$ factor due to pigeon-hole's
% principle.
% yu note: blowup not really \sqrt{S}, as the regret is not of
% \sqrt{T} order.

% Now consider Algorithm \ref{algorithm:VI_explore}.

Now, assume the initial state is $s_1$. Recall we have defined the
maximum reaching probability $\psi$ for state $s \in \cS_h$ as
\begin{equation*}
  \psi(s) = \max_{\mu, \nu}\P_{\mu, \nu}(s_h = s|s_1).
\end{equation*}
In Algorithm~\ref{algorithm:VI_explore}, we required an
$\text{EXPLORATION}(\epsilon)$ subroutine to output
$(\hat{\P}, \hat{r})$ that satisfies:
\begin{equation} \label{eq:condition_explore}
  \hat{r}(s, a, b) = r(s, a, b) \text{~and~} \norm{(\hat{\P} -
    \P)(\cdot|s, a, b)}_{\text{TV}} \le \epsilon 
  \text{~ for any~} (s, a, b) \text{~so that~} \psi(s) \ge \epsilon.
\end{equation}
In the following Lemma, we show that such a subroutine exists and can
be done with a bounded number of episodes and in polynomial time.
% \cnote{We can put exploration algorithm in appendix, and mainly
%   discuss the second step in the main paper.}
 
\begin{lemma}[Existence of $\text{EXPLORATION}(\epsilon)$ subroutine]
  There exists an algorithm that with high probability finds
  $(\hat{\P}, \hat{r})$ that satisfies Eq.\eqref{eq:condition_explore}
  within $\tlO(\frac{S^2AB \cdot \poly(H)}{\epsilon^3})$
  samples.~\yub{and poly time.}
\end{lemma}
\begin{proof}
We prove by construction. For each fixed state $s \in \S_h$, we can
design an artificial reward function $r(s, \cdot, \cdot) = 1$ and
$r(s', \cdot, \cdot) = 0$ for any $s' \neq s$. We can treat $\cA
\times \cB$ as new action space, and run for instance Q-learning-UCB
algorithm on it \cite{jin2018q}, which guarantees w.h.p to output a
collection of policy $\{\pi_\tau\}$ so that  
\begin{equation*}
  \frac{1}{t} \sum_{\tau=1}^t [V^\star(s_1) - V^{\pi_\tau}(s_1)] \le
  \tlO\paren{\sqrt{\frac{SAB \cdot \poly(H)}{t}}}.
\end{equation*}
We note for this special reward we designed, $V^\star(s_1) = \psi(s)$
and $V^{\pi_\tau}(s_1) = \P_{\pi_\tau}(s_h = s|s_1)$, so the above
bound implies that
\begin{equation} \label{eq:explore_state}
  \frac{1}{t} \sum_{\tau = 1}^t \P_{\pi_\tau}(s_h = s|s_1) \ge \psi(s) -
  \tlO\paren{\sqrt{\frac{SAB \cdot \poly(H)}{t}}} \ge \psi(s) -
  \frac{\epsilon}{2}
\end{equation}
where the last inequality holds if we pick $t = \tilde{\Theta}(\frac{SAB
  \cdot \poly(H)}{\epsilon^2})$.  

We can interpret~\eqref{eq:explore_state} as follows: if
$\psi(s) \ge \epsilon$, and we run a policy that is uniformly drawn
from this collection $\{\pi_\tau\}$, then we expect to visit state $s$
once every $\frac{2}{\epsilon}$ episode. For any
$(a,b)\in\mc{A}_h\times \mc{B}_h$, if $(s,a,b)$ is visited for at
least $\tlO(S/\epsilon^2)$ times, then we can estimate the reward and
transition model at $(s,a,b)$ accurately in the sense
of~\eqref{eq:condition_explore}.  Therefore, to
let~\eqref{eq:condition_explore} hold for this $s$ and all $(a,b)$, it
suffices to play with the aforementioned exploration policy for
$\tlO(AB \cdot S/\epsilon^2 \cdot 2/\epsilon)=\tlO(SAB/\epsilon^3)$
episodes.

Finally, we run this algorithm for any $s$, which can be finished in
$\tlO(S^2ABH/\epsilon^3)$ episodes, and are guaranteed
that~\eqref{eq:condition_explore} hold for all $s$ such that
$\psi(s)\ge\epsilon$ with high probability. This finishes the proof. 
\end{proof}

Clearly $\mdp(H, \cS, \cA, \cB, \hat{\P}, \hat{r})$ is also a valid
MDP. We denote the value function on this ``empirical'' MDP as
$\tilde{V}$ and $\tilde{Q}$. The following Lemma bounds the difference
between $V$ and $\tilde{V}$ uniformly for all policies $(\mu, \nu)$.
\begin{lemma}[Value function of approximate
  model] \label{lem:policy_evaluation} 
  Suppose condition~\eqref{eq:condition_explore} holds, then with high
  probability we have
  \begin{equation*}
    \abs{V_1^{\mu, \nu}(s_1) - \hat{V}_1^{\mu,
      \nu}(s_1)} \le 2\epsilon \cdot SABH^2 \quad \textrm{for
    all}~(\mu, \nu).
  \end{equation*}
\end{lemma}
\begin{proof}
  By standard decomposition (which can be proved by induction), we
  know % \cnote{this can be proved by induction.}
  \begin{align*}
    V_1^{\mu, \nu}(s_1) - \hat{V}_1^{\mu, \nu}(s_1)
    = \sum_{h} \sum_{s, a, b} p^{\mu, \nu}(s, a, b|s_1) \brac{(\P_h -
    \hat{\P}_h) \hat{V}_h (s, a, b)  + (r_h - \hat{r}_h)(s, a, b)}
    % = \sum_{h} \sum_{s, a, b} r_h(s, a, b) \P^{\mu, \nu}_h(s, a,
    % b|s_1) - \hat{r}_h(s, a, b) \hat{\P}^{\mu, \nu}_h(s, a, b|s_1) 
  \end{align*}
  Let $\cS_{c} = \{s \in \cS : \psi(s) \ge \epsilon \}$. Then, by
  condition Eq.\eqref{eq:condition_explore}, we have: 
  \begin{align*}
    & \quad |V_1^{\mu, \nu}(s_1) - \hat{V}_1^{\mu, \nu}(s_1)| \\
    & \le \epsilon SABH + \sum_{h} \sum_{s \in \cS_c}\sum_{a, b}  \brac{H
      \norm{(\P_h - \hat{\P}_h) \hat{V}_h (s, a, b)}_{TV}  + |(r_h -
      \hat{r}_h)(s, a, b)|} \\ 
    & \le 2\epsilon SABH^2.
  \end{align*}
  this finishes the proof.
  % For each fixed $h$, we have
  % \begin{align*}
  %   \sum_{s, a, b} r_h(s, a, b) \P^{\mu, \nu}_h(s, a, b|s_1) - \hat{r}_h(s, a, b) \hat{\P}^{\mu, \nu}_h(s, a, b|s_1)
% = \sum_{s, a, b}[r_h - \hat{r_h}](s, a, b) \P^{\mu, \nu}_h(s, a, b|s_1)
% + \sum_{h}
% \end{align*}
\end{proof}

We are now in position to prove the main theorem.
\begin{proof}[Proof of Theorem \ref{thm:polytime_guarantee}]
Since both $\inf$ and $\sup$ are contractive maps, by Lemma \ref{lem:policy_evaluation}, we have:
\begin{align*}
&|\inf_\nu V_1^{\hat{\mu}, \nu}(s_1) - \inf_\nu \hat{V}_1^{\hat{\mu}, \nu}(s_1)| \le 2\epsilon \cdot SABH^2\\
&|\sup_\mu V_1^{\mu, \hat{\nu}}(s_1) - \sup_\mu \hat{V}_1^{\mu, \hat{\nu}}(s_1)| \le 2\epsilon \cdot SABH^2
\end{align*}
Since $(\hat{\mu},\hat{\nu})$ are the Nash Equilibria for $(\hat{\P},
\hat{r})$, we have $\inf_\nu \hat{V}_1^{\hat{\mu}, \nu}(s_1) =
\sup_\mu \hat{V}_1^{\mu, \hat{\nu}}(s_1)$. This gives: 
\begin{align*}
\sup_\mu V_1^{\mu, \hat{\nu}}(s_1) - \inf_\nu V_1^{\hat{\mu}, \nu}(s_1)
\le& |\sup_\mu V_1^{\mu, \hat{\nu}}(s_1) - \sup_\mu \hat{V}_1^{\mu, \hat{\nu}}(s_1)| 
+ | \sup_\mu \hat{V}_1^{\mu, \hat{\nu}}(s_1) - \inf_\nu \hat{V}_1^{\hat{\mu}, \nu}(s_1)|\\
&+ | \inf_\nu \hat{V}_1^{\hat{\mu}, \nu}(s_1) - \inf_\nu V_1^{\hat{\mu}, \nu}(s_1)| \le 4\epsilon \cdot SABH^2.
\end{align*}
Therefore, if we run the explore then exploit algorithm for total $K$ episode, the total regret is:
\begin{equation*}
K_{\text{exp}} + 4\epsilon \cdot SABH^2 \times (K - K_{\text{exp}})
\end{equation*}
where $K_{\text{exp}} = \tlO(\frac{S^2AB \cdot \poly(H)}{\epsilon^3})$
is the number of episodes used to do pure exploration. By picking
$\epsilon = K^{-1/4}$ we finish the proof.
\end{proof}

==> Sections_arXiv/proof_turn.tex <==
%!TEX root = ../two-player.tex


% \section{Proof for Turn-based games}
\section{Proof of Theorem~\ref{theorem:ucbvi-regret}}

Let $(\pi_+^k,\pi_-^k)$ denote the policy at the beginning of episode
$k$, and $Q^{\set{\up, \low}, k}$ the upper and lower $Q$
estimates \emph{at the beginning of episode $k$}. Similarly let
% $N_{1,h}^k(x_h, a_h)$ and $N_{2,h}^k(x_h, a_h)$
$N_h(x_h,a_h)$
denote the state-action visitation counts before playing episode
$k$. Throughout
this section $C>0$ will denote an absolute constant that can vary from
line to line. We understand $1/\sqrt{n}$ as $1/\sqrt{n\vee 1}$ (so
that it equals one when $n=0$) unless otherwise specified.

\begin{lemma}[Valid upper and lower confidence bound]
  \label{lemma:ucb}
  Choosing $\beta_t=C\sqrt{H^2S\ell/t}$ for some absolute $C>0$, 
  with probability at least $1-\delta$ we have simultaneously for all 
  $k,h$ that
  \begin{enumerate}[(a)]
  \item Valid upper and lower confidence bounds: for all $(x_h,
    a_h)\in\mc{S}\times\mc{A}$
    \begin{equation*}
      Q_h^{\up,k}(x_h, a_h) \ge Q_h^{\star, \pi_-^k}(x_h, a_h)
      \ge Q_h^{\pi_+^k,\star}(x_h,a_h) \ge
      Q_h^{\low,k}(x_h, a_h).
    \end{equation*}
    % and similarly for all $(x_h,a_h)\in\mc{S}_2\times\mc{A}_2$
    % \begin{equation*}
    %   Q_h^{\up,k}(x_h, a_h) \ge Q_h^{\star,\pi_-^k}(x_h, a_h)
    %   \ge Q_h^{\pi_+^k, \star}(x_h, a_h)  \ge
    %   Q_h^{\low,k}(x_h, a_h).
    % \end{equation*}
  \item Small gap: for all $(x_h,a_h)$ % and $(x_h,a_h)$
    \begin{equation*}
      \begin{aligned}
        \left[Q_h^{\up, k} - Q_h^{\low, k}\right](x_h, a_h) \le
        \left[ \P_h(Q_h^{\up, k} - Q_h^{\low, k})(x_{h+1},
          \pi_{h+1}^k(x_{h+1}))\right](x_h, a_h) + 
        C\sqrt{\frac{H^2S\ell}{N_{1,h}^k(x_h, a_h)}}.
        % \\ & \left[Q_h^{\up, k} - Q_h^{\low, k}\right](x_h, a_h)
        % \le \left[ \P_h(Q_{1,h+1}^{\up, k} - Q_{1,h+1}^{\low, k})(x_{h+1},
        %   \pi_{1,h+1}^k(x_{h+1}))\right](x_h, a_h) +
        % C\sqrt{\frac{H^2S\ell}{N_{2,h}^k(x_h, a_h)}}.
      \end{aligned}
    \end{equation*}
  \end{enumerate}
\end{lemma}
\begin{proof}
  We first present a uniform convergence lemma.
  \begin{lemma}[Uniform convergence of functions]
    \label{lemma:uniform-convergence}
    Suppose $\P$ is a discrete distribution on $[S]$ and $\what{\P}_n$
    is its empirical estimate with $n$ samples, then we have
    \begin{equation*}
      \sup_{f:[S]\to [0,M]} \left| [\what{\P}_n - \P]f
      \right| \le CM\sqrt{\frac{S\log(n/\delta)}{n}}
    \end{equation*}
    for some absolute constant $C>0$ with probability at least
    $1-\delta$.
  \end{lemma}
  \yub{Proof TBA, standard Hoeffding + $\infty$-norm covering.}

  We now prove statement (a). For any fixed $k$, we establish the bound
  ``$\up,k \ge \star, \pi_-^k$''
  by induction on $h=H,H-1,\dots,1$ (and the
  other side ``$\pi_+^k,\star\ge \low,k$" follows similarly.) For the
  base case, we have that 
  \begin{equation*}
    Q_{H}^{\up,k}(x_h,a_h) \ge r_H(x_h,a_h) = 
    Q_{H}^{\pi_+^k,\star}(x_h,a_h)
  \end{equation*}
  always holds. For all the other cases, applying
  Lemma~\ref{lemma:uniform-convergence}, we have uniformly over all
  $k$, $h$, and $(x_h,a_h)$ that
  \begin{equation*}
    \begin{aligned}
      \left|
        [\what{\P}_{h}^k - \P_h]Q_h^{\up,k}(x_{h+1},
        \pi_{h+1}(x_{h+1}))](x_h,
        a_h) \right| \le CH\sqrt{\frac{S\log(N_{h}^k(x_h,
          a_h)/\delta')}{N_{h}^k(x_h, a_h)}} \le
      CH\sqrt{\frac{S\ell}{N_{1,h}^k(x_h, a_h)}},
      % \\
      % & \left|
      %   [\what{\P}_{2,h}^k - \P_h]Q_{1,h+1}^{\up,k}(x_{h+1},
      %   \pi_+(x_{h+1}))](x_h, a_h) \right| \le
      % CH\sqrt{\frac{S\log(N_{2,h}^k(x_h,
      %     a_h)/\delta')}{N_{1,h}^k(x_h, a_h)}} \le
      % CH\sqrt{\frac{S\ell}{N_{2,h}^k(x_h, a_h)}},     
    \end{aligned}
  \end{equation*}
  where we have set $\delta'=c\delta/(HSAK)$ and let
  $\ell=\log(HSAK/\delta)$. Therefore, choosing
  $\beta_t=C\sqrt{H^2S\ell/t}$, the update rule in
  Algorithm~\ref{algorithm:ucbvi} guarantees that
  \begin{equation*}
    \begin{aligned}
      & Q_h^{\up,k}(x_h, a_h) \ge r_h(x_h, a_h) +
      \left[\P_h\Q_{h+1}^{\up,k}(x_{h+1},
        \pi_{h+1}^k(x_{h+1}))\right](x_h, a_h)~~~\textrm{for all}~h\in
      \mc{H}_+ \\
      & Q_h^{\up,k}(x_h, a_h) \ge r_h(x_h, a_h) + \left[
        \P_hQ_{h+1}^{\up, k}(x_{h+1}, \pi_{h+1}^k(x_{h+1}))
      \right](x_h, a_h)\\
      & \quad\quad\quad
      = r_h(x_h, a_h) + \left[
        \P_h\left[ \max_{a_{h+1}'} Q_{h+1}^{\up, k}(x_{h+1}, a_{h+1}') 
        \right]\right](x_h, a_h)~~~\textrm{for all}~h\in\mc{H}_-,
    \end{aligned}
  \end{equation*}
  where the last equality follows from the fact that $h+1\in\mc{H}_+$
  and that $\pi_{h+1}^k\in\pi_+^k$ is defined as the argmax policy
  over $Q_{h+1}^{\up, k}$.

  Now, observe that the above recursion has exactly the
  form of the Bellman equation~\eqref{equation:bellman-star-2} for
  $Q^{\star,\pi_-^k}$ except having inequalities rather than
  equalities. Therefore, from the base case, we could inductively
  obtain that $Q_h^{\up, k}(x_h,a_h)\ge
  Q_h^{\star,\pi_-^k}(x_h,a_h)$
  % and $Q_h^{\up, k}(x_h,a_h)\ge Q_h^{\star,\pi_-^k}(x_h,a_h)$
  for all $h=H,H-1,\dots,1$ on the
  concentration event whose failure probability is at most $\delta$.

  Under the same concentration event, statement (b) follows by noting
  that
  \begin{equation*}
    \begin{aligned}
      Q_h^{\up,k}(x_h, a_h) \le r_h(x_h, a_h) +
      \left[\P_h\Q_{h+1}^{\up,k}(x_{h+1},
        \pi_{h+1}^k(x_{h+1}))\right](x_h, a_h)
      + C\sqrt{\frac{H^2S\ell}{N_{h}^k(x_h, a_h)}}
      % \\ & Q_h^{\up,k}(x_h, a_h) \le r_h(x_h, a_h) + \left[
      %   \P_hQ_{1,h+1}^{\up, k}(x_{h+1}, \pi_{1,h}^k(x_{h+1}))
      % \right](x_h, a_h) + C\sqrt{\frac{H^2S\ell}{N_{2,h}^k(x_h,
      %     a_h)}},
    \end{aligned}
  \end{equation*}
  and the corresponding lower bounds for $Q_{h}^{\low,k}$.
\end{proof}

\begin{lemma}[Gap propagation for $Q^{\up,k}-Q^{\low,k}$]
  \label{lemma:gap-propagation}
  With the bonus chosen as~\eqref{equation:bonus}, we have with
  probability at least $1-\delta$ that
  \begin{equation*}
    \begin{aligned}
      (Q_h^{\up,k} - Q_h^{\low,k})(x_h^k, a_h^k) \le
      (Q_h^{\up,k} - Q_h^{\low,k})(x_{h+1}^k, a_{h+1}^k) +
      C\sqrt{\frac{H^2S\ell}{N_{h}^k(x_h^k, a_h^k)}} + \eps_{h}^k,
      % \\
      % & (Q_h^{\up,k} - Q_h^{\low,k})(x_h^k, a_h^k) \le
      % (Q_{1,h+1}^{\up,k} - Q_{1,h+1}^{\low,k})(x_{h+1}^k, a_{h+1}^k) +
      % C\sqrt{\frac{H^2S\ell}{N_{2,h}^k(x_h^k, a_h^k)}} + \eps_{2,h}^k,
    \end{aligned}
  \end{equation*}
  where we have defined the error terms
  \begin{equation*}
    \eps_{h}^k \defeq [\P_h - \wt{\P}_{h}^k](Q_h^{\up,k} -
    Q_h^{\low,k})(x_h^k, a_h^k),
    % ~~~
    % \eps_{2,h}^k \defeq [\P_h - \wt{\P}_{2,h}^k](Q_{1,h+1}^{\up,k} -
    % Q_{1,h+1}^{\low,k})(x_h^k, a_h^k),
  \end{equation*}
  in which $\wt{\P}_{h}^k(x_h^k, a_h^k)\defeq \delta_{x_{h+1}^k}$
  % and $\wt{\P}_{2,h}^k(x_h^k,a_h^k)\defeq \delta_{x_{h+1}^k}$
  denote the observed transitions in episode $k$.
\end{lemma}
\begin{proof}
  The result follows straightforwardly from Lemma~\ref{lemma:ucb}(b)
  and replacing $\P_{h}$ with $\wt{\P}_{h}^k$ (and collecting the
  error terms into $\eps_h^k$.)
\end{proof}

We are now in position to prove the main theorem.

\begin{proof-of-theorem}[\ref{theorem:ucbvi-regret}]
For any fixed $k$, applying Lemma~\ref{lemma:ucb}(a), we have with
probability at least $1-\delta$
\begin{align*}
  & \quad \left[V_{1}^{\star,\pi_-^k} -
    V_{1}^{\pi_+^k,\star}\right](x_1^k)  = \max_{a_1'}
    Q_{1}^{\star,\pi_-^k}(x_1^k, a_1') -
    Q_{1}^{\pi_+^k,\star}(x_1^k, a_1^k) \\
  & \le \max_{a_1'} Q_{1}^{\up,k}(x_1^k, a_1') -
    Q_{1}^{\low, k}(x_1^k, a_1^k) = \left[Q_{1}^{\up,k} -
    Q_{1}^{\low,k}\right](x_1^k, a_1^k). 
\end{align*}
Now using the gap propagation in Lemma~\ref{lemma:gap-propagation}
repeatedly over $h=1,2,\dots,H$, the right hand side can be upper
bounded as
\begin{align*}
  \left[Q_{1}^{\up,k} - Q_{1}^{\low,k}\right](x_1^k, a_1^k) \le
  C\sqrt{H^2S\ell}\cdot \sum_{h=1}^H \frac{1}{\sqrt{N_{h}^k(x_h^k,
  a_h^k)}}  +
  \sum_{h=1}^H \eps_{h}^k.
\end{align*}
Summing over $k=1,2,\dots,K$ and re-arranging, we obtain
\begin{align*}
  & \quad \sum_{k=1}^K \left[Q_{1,1}^{\up,k} -
    Q_{1,1}^{\low,k}\right](x_1^k, a_1^k)
    \le C\sqrt{H^2S\ell} \cdot \sum_{h=1}^H \sum_{(x_h,a_h)}
    \sum_{n=0}^{N_{h}^K(x_h, a_h)} \frac{1}{\sqrt{n\vee 1}}
    % + \sum_{h=1}^H \sum_{(x_h,a_h)} 
    % \sum_{n=0}^{N_{2,h}^K(x_h, a_h)} \frac{1}{\sqrt{n\vee
    % 1}}\right)
    + \sum_{h=1}^H \sum_{k=1}^K \eps_{h}^k \\
    % + \sum_{h=1}^H \sum_{k=1}^K \eps_{2,h}^k
  & \le \underbrace{C\sqrt{H^2S\ell} \cdot \sum_{h=1}^H
    \sum_{(x_h,a_h)} \sqrt{N_{h}^K(x_h, a_h)}
    % + \sum_{h=1}^H \sum_{(x_h,a_h)} \sqrt{N_{2,h}^K(x_h,
    % a_h)}\right)
    }_{\rm I} +
    \underbrace{\sum_{h=1}^H \sum_{k=1}^K \eps_{h}^k
    % + \sum_{h=1}^H \sum_{k=1}^K \eps_{2,h}^k
    }_{\rm II}.
\end{align*}
For term I, we apply pigeonhole's principle: we have
$\sum_{h,(x_h,a_h)}N_{1,h}^K(x_h,a_h)=HK=T$ and there are $HSA$
summands, therefore
\begin{equation*}
  {\rm I} \le C\sqrt{H^2S\ell} \cdot \sqrt{HSAT}  =
  C\sqrt{H^3S^2AT\ell}.
\end{equation*}
For term II, we note that $\set{\eps_{h}^k}_{k=1}^K$ are martingale
difference sequences (as $\wt{\P}_{h}^k$ has conditional mean
$\P_{h}^k$ given all the information before) and satisfy
$|\eps_{h}^k|\le H$ almost surely. By
Azuma-Hoeffding's inequality~\yub{statement TBA}, we have uniformly
for all $h\in[H]$ that
\begin{equation*}
  \left|\sum_{k=1}^K \eps_{h}^k\right| \le
  C\sqrt{H^2K\log(H/\delta)} 
\end{equation*}
with probability at least $1-\delta$. Summing over $h$ gives
\begin{equation*}
  {\rm II} \le CH\sqrt{H^2K\log(H/\delta)} \le C\sqrt{H^4K\ell} =
  C\sqrt{H^3T\ell}. 
\end{equation*}
Combining the bounds for I and II (and rescaling $2\delta$ to
$\delta$), we have with probability at least $1-\delta$ that
\begin{align*}
  & \quad \sum_{k=1}^K \left[V_{1}^{\star,\pi_-^k} -
    V_{1}^{\pi_+^k,\star}\right](x_1^k) \\
  & \le \sum_{k=1}^K \left[Q_{1}^{\up,k} -
    Q_{1}^{\low,k}\right](x_1^k, a_1^k) \le {\rm I} + {\rm II} \le
  C(\sqrt{H^3S^2AT\ell} + 
  \sqrt{H^3T\ell}) \le C\sqrt{H^3S^2AT\ell}.
\end{align*}
This is the desired result.
\end{proof-of-theorem}




==> Sections_arXiv/simultaneous.tex <==
%!TEX root = ../two-player.tex



\section{Simultaneous games}

\begin{algorithm*}[ht]
   \caption{Upper-Lower Confidence Bound Value Iteration (Simultaneous Game Version)}
   \label{algorithm:ucbvi_sim}
\begin{algorithmic}[1]
   % \INPUT Parameter $\eta\in(0,1)$, $r_\star\in\Z_{>0}$, and $c>0$.
   \STATE {\bfseries Initialize:} for any $(x, a, b, h)$,
   $Q_{h}^\up(x,a, b)\setto H$, $Q_{h}^\low(x,a, b)\setto 0$,
   $N_{h}(x,a, b)\setto 0$.
   \FOR{episode $k=1,\dots,K$}
   % \STATE {\color{blue} \tt // Compute policy for both players}
   % \STATE Set $\pi_{1,h}(x_h) = \argmax_{a'} Q_1^\up(x_h, a')$ and
   % $\pi_{2,h}(x_h) = \argmin_{b'} Q_2^\low(x_h, b')$ for all
   % $h,x_h,x_h$. 
   \STATE Receive $x_1$.
   \FOR{step $h=H,H-1,\dots,1$}
   % \STATE {\color{blue} \tt // Player 2 update}
   \FOR{$(x, a, b)\in\cS\times\cA\times \cB$}
   \STATE $t=N_{h}(x, a, b)$;
   \STATE $Q_{h}^\up(x, a, b)\setto \min\set{r_h(x, a, b) +
   [\widehat{\P}_{h}^k V_{h+1}^\up](x, a, b) +
   \beta_t, H}$. \cnote{r may be unobserved yet.}
   \STATE $Q_{h}^\low(x, a, b)\setto \max\set{r_h(x, a, b) +
   [\widehat{\P}_{h}^k V_{h+1}^\low](x, a, b)
   - \beta_t, 0}$.
   \ENDFOR
   \FOR{$x \in \cS$}
   \STATE $(\mu_h(x), \nu_h(x)) \leftarrow \text{NASH\_GENERNAL\_SUM}(Q_h^\up(x, \cdot, \cdot), Q_h^\low(x_h, \cdot, \cdot))$.
   \STATE $V_h^\up(x) \leftarrow \mu_h(x)\trans Q_h^\up(x, \cdot, \cdot) \nu_h(x)$, \qquad $V_h^\low(x) \leftarrow \mu_h(x)\trans Q_h^\low(x, \cdot, \cdot) \nu_h(x)$.
   % \STATE $V_h^\low(x) = \mu_h(x)\trans Q_h^\low(x, \cdot, \cdot) \nu_h(x)$.
   \ENDFOR
   \ENDFOR
   \FOR{step $h=1,\dots, H$}
   % \STATE Compute $(\phi, \psi)=\text{NASH\_GENERNAL\_SUM}(Q^\up(x_h, \cdot, \cdot), Q^\low(x_h, \cdot, \cdot))$
   \STATE Take action $a_h \sim \mu_h(x_h)$, $b_h \sim \nu_h(x_h)$.
   % \STATE {\color{blue} \tt // Both players play}
   % \STATE If $h \in \cH_{+}$, take action $a_h=\pi_h(x_h) \defeq \argmax_{a} Q^\up(x_h, a)$
   % \STATE If $h \in \cH_{-}$, take action $a_h=\pi_h(x_h) \defeq \argmin_{a} Q^\low(x_h, a)$
   \STATE observe reward $r_h(x_h,a_h, b_h)$ and next state $x_{h+1}$.
   \STATE $N_{h}(x_h, a_h, b_h)\setto N_{h}(x_h, a_h, b_h) + 1$.
   % \STATE Take action $a_h=\pi_-(x_h)$, observe reward
   % $r_h(x_h,a_h)$ and next state $x_{h+1}$.
   % \STATE $N_{2,h}(x_h, a_h)\setto N_{2,h}(x_h, a_h) + 1$.
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm*}

Here, \text{NASH\_GENERNAL\_SUM} is a subroutine that takes two matrices $\mat{P}, \mat{Q} \in \R^{A\times B}$, and returns the Nash equilibrium $(\phi, \psi) \in \Delta_A \times \Delta_B$ for general sum game, which satisfies:
\begin{align*}
\phi\trans \mat{P} \psi = \max_{\tilde{\phi}} \tilde{\phi}\trans \mat{P} \psi, \qquad \phi\trans \mat{Q} \psi = \min_{\tilde{\psi}} \phi\trans \mat{Q} \tilde{\psi},
\end{align*}
\cnote{maybe we need to consider error version of finding Nash?}





\subsection{Main Result}


\begin{theorem} \label{thm:main_sim}
For two-player simultanoues MDP \cnote{better name}, with probability at least $1-p$, the regret of Algorithm \ref{algorithm:ucbvi_sim} is at most $\cO(\sqrt{H^3S^2ABT\iota})$, where $\iota = \log(SABT/p)$.
\end{theorem}


\paragraph{Notation:} To be clear from the context, we denote the upper bound and lower bound $Q^\up$ and $Q^\low$ computed at the $k$-th episode as $Q^{\up, k}$ and $Q^{\low, k}$, and policies computed and used at the $k$-th episode as $\mu_k$ and $\nu_k$.

\paragraph{Choice of bonus:} $\beta_t = c\sqrt{SH^2\iota/t}$ for sufficient large absolute constant $c$.

\begin{lemma}[ULCB]\label{lem:ULCB_sim}
With probability at least $1-p$, we have following bounds for any $(x, a, b, h, k)$:
% $\in \cS\times\cA\times\cB\times[H]\times[K]$
\begin{align}
&V_h^{\up, k}(x) \ge \sup_{\mu} V_h^{\mu, \nu_k}(x),  &Q_h^{\up, k}(x, a, b) \ge& \sup_{\mu} Q_h^{\mu, \nu_k}(x, a, b) \label{eq:ucb_sim}\\
&V_h^{\low, k}(x) \le \inf_{\nu} V_h^{\mu_k, \nu}(x), &Q_h^{\low, k}(x, a, b) \le& \inf_{\nu} Q_h^{\mu_k, \nu}(x, a, b) \label{eq:lcb_sim}
\end{align}
\end{lemma}
\begin{proof}
By symmetry, we only need to prove the statement \eqref{eq:ucb_sim}. For each fixed $k$, we prove this by induction from $h=H+1$ to $h=1$. For base case, we know at the $(H+1)$-th step, 
$V_{H+1}^{up, k}(x) = \sup_{\mu} V_{H+1}^{\mu, \nu_k}(x) = 0$.

Now, assume the left inequality in \eqref{eq:ucb_sim} holds for $(h+1)$-th step, for the $h$-th step, we first recall the updates for $Q$ functions respectively:
\begin{align*}
Q_{h}^{\up, k}(x, a, b) = & \min\set{r_h(x, a, b) +
   [\widehat{\P}_{h}^k V_{h+1}^{\up, k}](x, a, b) +
   \beta_t, H}\\
\sup_{\mu} Q_h^{\mu, \nu_k}(x, a, b)
=& r_h(x, a, b) + [\P_{h} \sup_{\mu}V_{h+1}^{\mu, \nu_k}](x, a, b)
\end{align*}
In case of $Q_{h}^{\up, k}(x, a, b) = H$, the right inequality in \eqref{eq:ucb_sim} clearly holds. Otherwise, we have:
\begin{align*}
Q_{h}^{\up, k}(x, a, b) - \sup_{\mu} Q_h^{\mu, \nu_k}(x, a, b)
=& [\widehat{\P}_{h}^k V_{h+1}^{\up, k}](x, a, b) - [\P_{h}^k \sup_{\mu}V_{h+1}^{\mu, \nu_k}](x, a, b) +  \beta_t\\
=& [\widehat{\P}_{h}^k (V_{h+1}^{\up, k} - \sup_{\mu}V_{h+1}^{\mu, \nu_k})](x, a, b) - [(\widehat{\P}_{h}^k -\P_{h}) \sup_{\mu}V_{h+1}^{\mu, \nu_k}](x, a, b) +  \beta_t
\end{align*}
Since $\widehat{\P}_{h}^k$ perserves the positivity, by induction assumption, we know the first term is positive. By Lemma \ref{lem:uniform_concern_sim}, we know the second term $\ge -\beta_t$. This finishes the proof of the right inequality in \eqref{eq:ucb_sim}.

To prove the left inequality in \eqref{eq:ucb_sim}, again recall the updates for $V$ functions respectively:
\begin{align*}
V_{h}^{\up, k}(x) = & \mu^k_h(x)\trans Q_h^{\up, k}(x, \cdot, \cdot) \nu^k_h(x) = \max_{\phi \in \Delta_\cA} \phi\trans Q_h^{\up, k}(x, \cdot, \cdot) \nu^k_h(x) \\
\sup_{\mu} V_h^{\mu, \nu_k}(x) = &\max_{\phi \in \Delta_\cA} \phi\trans [\sup_{\mu} Q_h^{\mu, \nu^k}(x, \cdot, \cdot)] \nu^k_h(x)
\end{align*}
where the first equation is by the definition of policy $\mu_k$ the algorithm picks. Therefore:
\begin{equation*}
V_{h}^{\up, k}(x) - \sup_{\mu} V_h^{\mu, \nu_k}(x)
\ge \max_{\phi \in \Delta_\cA} \phi\trans [Q_h^{\up, k} - \sup_{\mu} Q_h^{\mu, \nu^k}](x, \cdot, \cdot) \nu^k_h(x) \ge 0.
\end{equation*}
This finishes the proof.
\end{proof}

% \begin{lemma}[Uniform Concentration]\label{lem:uniform_concern_sim}
% Consider value function class $\mathcal{V} = \{V: \cS\times\cA\times\cB \rightarrow \R| \forall (x, a, b), V(x, a, b)\in[0, H] \}$. 
% % Suppose we have encountered $(x, a, b)$ for $t$ times, and $\hat{\P}$ is the empirical transition matrix. Then, 
% There exists an absolute constant $c$, with probability at least $1-p$, we have:
% \begin{equation*}
% \forall V\in \mathcal{V}, \forall (x, a, b, k, h), \quad |[(\hat{\P}^k_h - \P_h)V](x, a, b)| \le c\sqrt{SH^2\iota/N^k_h(x, a, b)}
% \end{equation*}
% \end{lemma}

\begin{lemma}[Uniform Concentration]\label{lem:uniform_concern_sim}
Consider value function class $\mathcal{V} = \{V: \cS\times\cA\times\cB \rightarrow \R| \forall (x, a, b), V(x, a, b)\in[0, H] \}$. 
% Suppose we have encountered $(x, a, b)$ for $t$ times, and $\hat{\P}$ is the empirical transition matrix. Then, 
There exists an absolute constant $c$, with probability at least $1-p$, we have:
\begin{equation*}
\forall V\in \mathcal{V}, \forall (x, a, b, k, h), \quad |[(\hat{\P}^k_h - \P_h)V](x, a, b)| \le c\sqrt{SH^2\iota/N^k_h(x, a, b)}
\end{equation*}
\end{lemma}

\begin{proof}
This is standard from Hoeffding bound and $\epsilon$-net argument. \cnote{to be filled in more details.}
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:main_sim}]
By Lemma \ref{lem:ULCB_sim}, we know the regret,
\begin{equation*}
\text{Regret}(K) = \sum_{k=1}^K \left[\sup_{\mu}\sind{V}{\mu, \nu_k}{1} (\ind{x}{k}{1}) - \inf_{\nu}\sind{V}{\mu_k, \nu}{1} (\ind{x}{k}{1})\right] 
\le \sum_{k=1}^K [V_1^{\up, k}(\ind{x}{k}{1})  - V_1^{\low, k}(\ind{x}{k}{1})]
\end{equation*}
On the other hand, by the updates in Algorithm \ref{algorithm:ucbvi_sim}, we have:
\begin{align*}
[V_h^{\up, k} - V_h^{\low, k}](\ind{x}{k}{h})
=& \mu^k_h(x^k_h)\trans [Q_h^{\up, k} - Q_h^{\low, k}](x^k_h, \cdot, \cdot) \nu^k_h(x^k_h), \\
=& [Q_h^{\up, k} - Q_h^{\low, k}](x^k_h, a^k_h, b^k_h) + \xi^k_h\\
\le & [\widehat{\P}_{h}^k (V_{h+1}^{\up, k} - V_{h+1}^{\low, k})](x^k_h, a^k_h, b^k_h) + 2\beta_h^k + \xi_h^k \\
\le & \P (V_{h+1}^{\up, k} - V_{h+1}^{\low, k})](x^k_h, a^k_h, b^k_h) + 4\beta_h^k + \xi_h^k\\
= & [V_{h+1}^{\up, k} - V_{h+1}^{\low, k})](\ind{x}{k}{h+1}) + 4\beta_h^k + \xi_h^k + \zeta_h^k
\end{align*}
the last inequality is due to Lemma \ref{lem:uniform_concern_sim}. $\xi_h^k$ and $\zeta_h^k$ are defined as
\begin{align*}
\xi_h^k =& \E_{a \sim \mu^k_h(x^k_h), b\sim \nu^k_h(x^k_h)} [Q_h^{\up, k} - Q_h^{\low, k}](x^k_h, a, b)  - [Q_h^{\up, k} - Q_h^{\low, k}](x^k_h, a^k_h, b^k_h)\\
\zeta_h^k =& \E_{x \sim \P(\cdot|x^k_h, a^k_h, b^k_h)} (V_{h+1}^{\up, k} - V_{h+1}^{\low, k})](x) - [V_{h+1}^{\up, k} - V_{h+1}^{\low, k})](\ind{x}{k}{h+1})
\end{align*}
Both $\xi_h^k$ and $\zeta_h^k$ are martingale difference sequence, with probability $1-p$, we have:
\begin{equation*}
\sum_{k, h} \xi_h^k \le \cO(\sqrt{HT\iota}), \quad \sum_{k, h} \zeta_h^k \le \cO(\sqrt{HT\iota}).
\end{equation*}
Therefore, by our choice of bonus $\beta_t$ and the Pigeonhole principle, we have
\begin{align*}
\sum_{k=1}^K [V_1^{\up, k}(\ind{x}{k}{1})  - V_1^{\low, k}(\ind{x}{k}{1})]
\le \sum_{k, h} (4\beta^k_h + \xi^k_h + \zeta^k_h)\le \cO(\sqrt{H^3S^2ABT\iota})
\end{align*}
This finishes the proof.
\end{proof}


% \subsection{Mirror descent for one-step simultaneous game}
% \cnote{Cite the mirror descent result for simultaneous game.}



% We now present our mirror descent based algorithm for one-step
% turn-based games. Define the loss estimates
% \begin{align}
%     & \wt{Q}_1^k(x_1^k, a) \defeq 2 - 
%     \frac{\indic{a_1^k=a}}{\pi_1^k(a|x_1^k)} \cdot \brac{2 - (r(x_1^k, a) +
%       r(x_2^k, a_2^k))}~~~\textrm{for
%       all}~a\in\mc{A}, \label{equation:q1-estimate} \\ 
%     & \wt{Q}_2^k(x_2^k, a) \defeq 1 - 
%     \frac{\indic{a_2^k=a}}{\pi_2^k(a|x_2^k)} \cdot \brac{1 - r(x_2^k,
%       a)}~~~\textrm{for all}~a\in\mc{A}. \label{equation:q2-estimate}
% \end{align}
% The full algorithm is described in
% Algorithm~\ref{algorithm:mirror-descent}.

% \begin{algorithm*}[ht]
%    \caption{Mirror descent for one-step turn-based game}
%    \label{algorithm:mirror-descent}
%    \begin{algorithmic}
%      \INPUT Learning rate $\eta$.
%      \STATE {\bf Initialize}: Set $(\pi_+,\pi_-)$ to be uniform:
%      $\pi_{h}(a|x)=\frac{1}{A}$ for all $(x,a,h)$.
%      % $\pi_-(b|y)=\frac{1}{B}$ for all $(y,b)$.
%      \FOR{episode $k=1,\dots,K$}
%      % \STATE {\color{blue} \tt // Both players play}
%      \FOR{step $h=1,2$}
%      \STATE Receive $x_h$.
%      \STATE Play action $a_h\sim \pi_h(\cdot|x)$ and observe
%      reward $r_h(x,a)$.
%      \ENDFOR
%      % \STATE Receive $y^k$ for player 2.
%      % \STATE Play action $b^k\sim\pi_-(\cdot|y^k)$ and observes
%      % reward $r(y^k,b^k)$.
%      % \STATE {\color{blue} \tt // Both players update}
%      \STATE Compute $\set{\wt{Q}_1^k(x_1^k,a)}_{a\in\mc{A}}$ according
%      to~\eqref{equation:q1-estimate} and update
%      $$\pi_1^{k+1}(a|x_1^k)  \propto\pi_1^k(a|x_1^k) \cdot \exp(\eta_+
%      \wt{Q}_1^k(x_1^k,a)).$$
%      \STATE Compute $\set{\wt{Q}_2^k(x_2^k, a)}_{a\in\mc{A}}$
%      according to~\eqref{equation:q2-estimate} and update
%      $$\pi_2^{k+1}(a|x_2^k) \propto 
%      \pi_2^{k}(a|x_2^k) \cdot \exp(-\eta_- \wt{Q}_2^k(x_2^k, a)).$$
%      \ENDFOR
%    \end{algorithmic}
% \end{algorithm*}

==> Sections_arXiv/turn-based.tex <==
%!TEX root = ../two-player.tex


\section{Turn-based games}
% \paragraph{Worst-case opponent and strong regret}
% For any maximizing policy $\mu$, its worst-case
% opponent is defined as
% $\pi_-^\star(\pi_+) \defeq \argmin_{\pi_-'} V^{\pi_-',
%   \pi_+'}$. Similarly define $\pi_+^\star(\pi_-) \defeq
% \argmax_{\pi_+'} V^{\pi_+',\pi_-}$. For convenience we will use
% $V^{\star,\pi_-},Q^{\star,\pi_-}$ to denote
% $V^{\pi_+^\star(\pi_-),\pi_-},Q^{\pi_+^\star(\pi_-),\pi_-}$ for any
% $\pi_-$, and similarly $V^{\pi_+,\star},Q^{\pi_+,\star}$ to denote
% $V^{\pi_+,\pi_-^\star(\pi_+)},Q^{\pi_+,\pi_-^\star(\pi_+)}$. 

% The Q function $Q_h^{\star, \pi_-}$ satisfies the following Bellman
% equations 
% \begin{equation}
%   \label{equation:bellman-star-2}
%   \begin{aligned}
%     & Q_h^{\star, \pi_-}(x_h, a_h) = r_h(x_h, a_h) +
%     \P_h\left[Q_h^{\star, \pi_-}(x_h,
%       \pi_{h}(x_h))\right](x_h, a_h)~~~\textrm{for all}~h\in
%     \mc{H}_+,\\
%     & Q_h^{\star, \pi_-}(x_h, a_h) = r_h(x_h, a_h) +
%     \P_h\left[\max_{a_{h+1}'} Q_{h+1}^{\star, \pi_-}(x_{h+1},
%     a_{h+1}')\right](x_h, a_h)~~~\textrm{for all}~h\in\mc{H}_-. 
%   \end{aligned}
% \end{equation}
% Similarly we also have
% \begin{equation}
%   \label{equation:bellman-1-star}
%   \begin{aligned}
%     & Q_h^{\pi_+, \star}(x_h, a_h) = r_h(x_h, a_h) +
%     \P_h\left[\min_{a_h'} Q_h^{\pi_+, \star}(x_h, a_h')\right](x_h,
%     a_h)~~~\textrm{for all}~h\in\mc{H}_+, \\
%     & Q_h^{\pi_+, \star}(x_h, a_h) = r_h(x_h, a_h) +
%     \P_h\left[Q_{1,h+1}^{\pi_+, \star}(x_{h+1},
%       \pi_{h+1}(x_{h+1}))\right](x_h, a_h)~~~\textrm{for
%       all}~h\in\mc{H}_-.
%   \end{aligned}
% \end{equation}

% For any algorithm that deploys
% policy $(\pi_+^k, \pi_-^k)$ in episode $k$, we define its regret as
% \begin{equation}
%   \Reg(K) \defeq \sum_{k=1}^K V^{\star, \pi_-^k}(x_1^k)
%   - V^{\pi_+^k, \star}(x_1^k).
% \end{equation}

\paragraph{Regret}
We will also consider a weaker notion of regret, in which for both
players, we only compare the deployed policies against a same opponent
policy over all episodes: \yub{Cite Auer et al 2001.}
\begin{equation}
  \Reg(K) \defeq \max_{\mu} \sum_{k=1}^K V^{\mu,
    \nu^k}(x_1^k) - \min_{\nu} \sum_{k=1}^K V^{\mu^k,
    \nu}(x_1^k).
\end{equation}

\subsection{Algorithm: Upper-Lower Confidence Bound Value Iteration}
Our main algorithm is presented in
Algorithm~\ref{algorithm:ucbvi}.~\yub{At a high level, our algorithm
  does BLAH BLAH...}

We further set the bonus to be
\begin{equation}
  \label{equation:bonus}
  \beta_t = c\sqrt{\frac{H^2S\ell}{t}},
\end{equation}
where $\ell\defeq \log(HS(A+B)T/\delta)$ is a log factor and $c>0$ is a
universal constant.

% Define $\cH_{-}$ be the set of min-player steps, and $\cH_{+}$ be the set of max-player steps. $\pi_{+} = \{ \pi_h | h \in \cH_{+}\}$, $\pi_{-} = \{ \pi_h | h \in \cH_{-}\}$.
% \begin{equation}
%   \Reg(K) \defeq \sum_{k=1}^K \max_{\pi_{+}}V_1^{\pi_+, \pi_-^k}(x_1^k)
%   - \min_{\pi_-}V_1^{\pi_+^k, \pi_-}(x_1^k).
% \end{equation}

\begin{algorithm*}[ht]
   \caption{Upper-Lower Confidence Bound Value Iteration}
   \label{algorithm:ucbvi}
\begin{algorithmic}
   % \INPUT Parameter $\eta\in(0,1)$, $r_\star\in\Z_{>0}$, and $c>0$.
   \STATE {\bfseries Initialize:} for any $(x, a, h)$,
   $Q_{h}^\up(x,a)\setto H$, $Q_{h}^\low(x,a)\setto 0$,
   $N_{h}(x,a)\setto 0$.
   \FOR{episode $k=1,\dots,K$}
   % \STATE {\color{blue} \tt // Compute policy for both players}
   % \STATE Set $\pi_{1,h}(x_h) = \argmax_{a'} Q_1^\up(x_h, a')$ and
   % $\pi_{2,h}(x_h) = \argmin_{b'} Q_2^\low(x_h, b')$ for all
   % $h,x_h,x_h$. 
   \STATE Receive $x_1$.
   \FOR{step $h=1,\dots, H$}
   % \STATE {\color{blue} \tt // Both players play}
   \STATE If $h \in \cH_{\max}$, take action $a_h=\pi_h(x_h) \defeq \argmax_{a} Q^\up(x_h, a)$
   \STATE If $h \in \cH_{\min}$, take action $a_h=\pi_h(x_h) \defeq \argmin_{a} Q^\low(x_h, a)$
   \STATE observe reward $r_h(x_h,a_h)$ and next state $x_{h+1}$.
   \STATE $N_{h}(x_h, a_h)\setto N_{h}(x_h, a_h) + 1$.
   % \STATE Take action $a_h=\pi_-(x_h)$, observe reward
   % $r_h(x_h,a_h)$ and next state $x_{h+1}$.
   % \STATE $N_{2,h}(x_h, a_h)\setto N_{2,h}(x_h, a_h) + 1$.
   \ENDFOR
   \FOR{step $h=H,H-1,\dots,1$}
   % \STATE {\color{blue} \tt // Player 2 update}
   \FOR{$(x, a)\in\mc{S}\times\mc{C}_h$}
   \STATE $t=N_{h}(x, a)$;
   \STATE $Q_{h}^\up(x, a)\setto \min\set{r_h(x, a) +
   [\widehat{\P}_{h}^k Q^\up(x', \pi_{h+1}(x'))](x, a) +
   \beta_t, H}$.
   \STATE $Q_{h}^\low(x, a)\setto \max\set{r_h(x,a) +
   [\widehat{\P}_{h}^k Q^\low(x', \pi_{h+1}(x'))](x, a)
   - \beta_t, 0}$.
   \ENDFOR
   \ENDFOR
   \ENDFOR
\end{algorithmic}
\end{algorithm*}

\subsection{Main Result}
\begin{theorem}
  \label{theorem:ucbvi-regret}
  With probability at least $1-\delta$,
  Algorithm~\ref{algorithm:ucbvi} achieves regret bound $\Reg(K) \le
  O(\sqrt{H^3S^2AT})$.
\end{theorem}

